Bidirectional Cross-Modal Knowledge Exploration for Video Recognition with Pre-trained Vision-Language Models

Vision-language models (VLMs) pre-trained on large-scale image-text pairs have demonstrated impressive transferability on various visual tasks. Transferring knowledge from such powerful VLMs is a promising direction for building effective video recognition models. However, current exploration in this field is still limited. We believe that the greatest value of pre-trained VLMs lies in building a bridge between visual and textual domains. In this paper, we propose a novel framework called BIKE, which utilizes the cross-modal bridge to explore bidirectional knowledge: i) We introduce the Video Attribute Association mechanism, which leverages the Video-to-Text knowledge to generate textual auxiliary attributes for complementing video recognition. ii) We also present a Temporal Concept Spotting mechanism that uses the Text-to-Video expertise to capture temporal saliency in a parameter-free manner, leading to enhanced video representation. Extensive studies on six popular video datasets, including Kinetics-400 & 600, UCF-101, HMDB-51, ActivityNet and Charades, show that our method achieves state-of-the-art performance in various recognition scenarios, such as general, zero-shot, and few-shot video recognition. Our best model achieves a state-of-the-art accuracy of 88.6% on the challenging Kinetics-400 using the released CLIP model. The code is available at https://github.com/whwu95/BIKE .

==> sections/03_method/st_attn.tex <==
\subsection{Learning Salient Representation}
In addition to the auxiliary knowledge mentioned above, we also attempt to capture spatio-temporal saliency to enhance the video representations.
To obtain the video representation based on a pre-trained image model, the typical pipeline can be divided into two steps: first, we employ the image model to extract the spatial embedding (\eg, [CLS] token) of each frame, and then the embeddings of these frames are temporally aggregated (\eg, mean pooling) to yield video-level representation.
Therefore, we explore learning salient representations from both spatial and temporal aspects in the following.

\noindent\textbf{Spatial Saliency Perception.}
With the visual transformer serving as the backbone, it is common practice to utilize the final [CLS] token as the embedding for each sampled frame, which is a form of global spatial information.
However, the local and fine-grained spatial signals may also be valuable for distinguishing different videos.
% However, this may cause spatial details to be ignored, making it difficult for the model to distinguish fine-grained information from different videos. 
Thus, we design a Spatial Saliency Perception (SSP) mechanism to select salient patches as the complement to the global embedding (\ie, [CLS] token). 
Specifically,

Formally,
% 因此我们提出了对于这个帧选取topk个重要的patch，然后与cls_token进行结合，既包含了这个帧的全局信息也包含了这个帧的重要信息。选取topk个patch策略:由于多头注意力权重分数代表一个patch与另一个patch的相似度大小，那么相似度越高，那么这两个patch关联性越大，表明越重要，根据这个现象，我们对视频帧经过visual transformer后得到不同层的注意力权重分数，然后进行求mean，得到一个整体的注意力权重分数，然后再对所有patch进行求mean得到所有patch的平均权重分数，这个平均权重分数，即代表这个patch对所有patch的重要程度，权重分数越大，也即是对所有patch的重要性越高，也即是对这个帧的重要性越大，然后根据平均注意力权重分数选取topk个比较重要的patch_token进行求mean，再与cls_token进行结合，得到一个即代表这个帧的全局信息也代表这个帧的重要信息

xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx 

\noindent\textbf{Temporal Saliency Aggregation.} Mean pooling is a straightforward and widely used technique to aggregate the frame embeddings to get the final video representation. 
Instead of treating each video frame equally as in mean pooling, we propose a parameter-free solution to utilize the pre-aligned visual and textual semantics offered by the VLM (\eg, CLIP~\cite{CLIP}) to capture temporal saliency for video feature aggregation. 
% 这里我们巧妙地利用单词特征和帧特征的相似度作为时序的显著性，利用这个显著性对帧进行聚合。
The pre-trained VLM can encode each video or category name separately, and output two set of embeddings: 
$\{\mathbf{v}_t \in \mathbb{R}^{d} | t=1,2,\cdots,T\}$ is a set of frame embeddings, where $T$ is the number of sampled frames, and $\{\mathbf{t}_n \in \mathbb{R}^{d}|n=1,2,\cdots,N\}$ is a set of word embeddings, where $N$ is the number of words in the class name.
Then we can utilize the similarity between words and frames as temporal saliency:

\begin{equation}
\mathcal{S}_{t,n}= \dfrac{\exp({\mathbf{v}_t}^\mathsf{T}\mathbf{t}_n/\tau)}{\sum_{n=1}^N \exp({\mathbf{v}_t}^\mathsf{T} \mathbf{t}_n/\tau)}, t \in [1, T], n \in [1, N],
\label{eq:softmax}
\end{equation}
where $\tau$ is the temperature of this softmax function.
% and $s_{i,j}$ computes similarity between the frame embedding $e_i^V$ and the word embedding $e_j^T$ as
% \begin{equation}
%     s_{i,j} = (\mathbf{v}_i)^{\mathsf{T}}(\mathbf{t}_j), i \in [1, T], j \in [1, N].
% \end{equation}
Then we utilize the temporal saliency to aggregate these frame embeddings: 
\begin{equation}
    \mathbf{e_v} = \frac{1}{N} \sum_{n=1}^N \mathbf{a}_n = \frac{1}{N} \sum_{n=1}^N \sum_{t=1}^T \mathbf{v}_t \mathcal{S}_{t,n},
\end{equation}
 $\mathbf{a}_n \in \mathbb{R}^{d}$ is the aggregated video representation using the similarity with $n^{th}$ word, and $\mathbf{e_v} \in \mathbb{R}^{d}$ is the final average video representation.
